Hybrid Solver for the Radiative Transport Equation Using Finite Volume and Discontinuous Galerkin

We propose a hybrid spatial discretization for the radiative transport equation that combines a second-order discontinuous Galerkin (DG) method and a second-order finite volume (FV) method. The strategy relies on a simple operator splitting that has been used previously to combine different angular discretizations. Unlike standard FV methods with upwind fluxes, the hybrid approach is able to accurately simulate problems in scattering dominated regimes. However, it requires less memory and yields a faster computational time than a uniform DG discretization. In addition, the underlying splitting allows naturally for hybridization in both space and angle. Numerical results are given to demonstrate the efficiency of the hybrid approach in the context of discrete ordinate angular discretizations and Cartesian spatial grids.

==> sections/discontGal.tex <==
\section{Discontinuous Galerkin}\label{app:DG}
For a single ordinate $\Omega_k$, \eqref{eq:RTEa} can be written as
\begin{equation}\label{RTsteadysingle}
\cL_k\psi_k=(\cS\cP\bspsi)_k+q_k,
\end{equation}
when $\epsilon = 1$, $\sigma_{\rm{s}}=\sigma_{\rm{t}}-\sigma_{\rm{a}}$, and 
\begin{subequations}
\begin{align}\label{eq:TDOp}
\cP\colon& \bbR^{K}\to\bbR,\quad\text{s.t.}\quad \cP_{k}=w_k,\\
\cS\colon& \bbR\to\bbR^{K},\quad\text{s.t.}\quad\cS_{k}=\frac{\sigma_{\rm{s}}}{4\pi}.
\end{align}
\end{subequations}

We discretize \eqref{RTsteadysingle} using the discontinuous Galerkin (DG) method \cite{DGM} with upwind numerical fluxes. Our presentation follows \cite{Crockatt} closely.We assume $X$ is a rectangular domain and create a uniform partition $\cT_h$ of $X$ with rectangular cells $\cK$ of maximum length $h$ and a fixed aspect ratio. We let $\cE_h$ be the collection of interior edges in $\cT_h$, and for each $e\in\cE_h$, we let $n_e$ be the associated normal vector with orientation chosen beforehand. 

Let $V_h$ be a finite dimensional function space over the spatial variable such that for each $v\in V_h$, $v|_{\cK}$ is a polynomial for each $\cK\in\cT_h$. The DG method is then to find $\psi_k^h\in V_h$ for each $i\le K$ satisfying
\begin{equation}\label{DGeq1}
\cB_k^h(\psi_k^h,v^h)=\bar{\cB}^{h}(\cS\cP\bspsi^h,v^h)+\cA_k^h(v^h),\quad \forall\ v^h\in V_h,
\end{equation}
where $\bspsi^h=[\psi_1^h,\psi_2^h,\ldots,\psi_{K}^h]^T$. The bilinear and linear forms are given by
\begin{subequations}
\begin{align}
\label{eqBLF1}\cB_k^h(u,v)=&-\sum_{\cK\in\cT_h}\int_{\cK}\left(\Omega_k\cdot\nabla_xv\right)u\ dx+\sum_{\cK\in\cT_h}\int_{\cK}\Lambda_{k,k}vu\ dx\\
\nonumber&-\sum_{e\in\cE_h}\int_e(\Omega_k\cdot n_e)[v]\widehat{u}\ dx+\sum_{e\in\partial X_k^+}\int_e(\Omega_k\cdot n_e)v^-u^-\ ds,\\
\bar{\cB}^h(u,v)&=\sum_{\cK\in\cT_h}\int_{\cK}vu\ dx,\\
\cA_k^h(v)&=\sum_{\cK\in\cT_h}\int_{\cK}q_kv\ dx-\sum_{e\in\partial X_k^-}\int_e\left(\Omega_k\cdot n_e\right)\psi_k^Bv^-\ dx,
\end{align}
\end{subequations}
where $\psi_k^B=\psi_k^B(x)$ is the inflow on $\partial X_k^-$,
\begin{equation}
v^{\pm}(x)=\lim_{\epsilon\to 0^+}v(x\pm\epsilon n_e),\quad [v]=v^+-v^-,\quad\text{and}\quad\widehat{u}_k=\lim_{\epsilon\to0^+}u_k(x-\epsilon\Omega_k).
\end{equation}
To formulate a matrix equation from \eqref{DGeq1}, let $\bb_h$ be a vector whose components form a basis of $V_h$, and let $\bsalpha_{k}^h$ be a real vector such that $\psi_k^h=\bb_h^T\bsalpha_k^h$. Then \eqref{DGeq1} can be reduced to
\begin{equation}\label{DGeq2}
\cL^h\bsPsi^h=\cS^h\cP^h\bsPsi^h+\bq^h,
\end{equation}
where $\cL^h$ is a block diagonal matrix with blocks $\{\cL_k^h\}_{k=1}^{K}$, $(\bsPsi^h)^T=\left[(\bsalpha_1^h)^T,(\bsalpha_2^h)^T,\ldots,(\bsalpha_{K}^h)^T\right]$, $(\bq^h)^T=\left[(\bq_1^h)^T,(\bq_2^h)^T,\ldots,(\bq_{K}^h)^T\right]$, $\cS^h=\cS\otimes\bar{\cS}^h$, and
\begin{equation}
\cL_k^h=\cB_k^h(\bb_h^T,\bb_h),\quad \bq_k^h=\cA_k^h(\bb_h),\quad \bar{\cS}^h=\bar{\cB}^h(\bb_h^T,\bb_h),\quad \cP^h\bsPsi^h=\sum_{k=1}^{K}w_k\bsalpha_k^h.
\end{equation}

==> sections/finitevolume.tex <==
\section{Finite Volume}\label{app:FV}
Suppose domain $X$ is partitioned into uniform cells $[x_{i-1/2},x_{i+1/2}]\times[y_{j-1/2},y_{j+1/2}]$ where $1\le i\le I$, $1\le j\le J$, $(x_i,y_j)$ is the center of each cell and $\Delta x_i=x_{i+1/2}-x_{i-1/2}$ and $\Delta y_j=y_{j+1/2}-y_{j-1/2}$ for all $i,j$. Define the cell-average angular flux $\psi_{k,i,j}$ by
\begin{equation}\label{eq:cellavg}
    \psi_{k,i,j} = \frac{1}{\Delta x_i\Delta y_j}\int_{x_{i-1/2}}^{x_{i+1/2}}\int_{y_{j-1/2}}^{y_{j+1/2}}\psi_k(x,y)\ dx\ dy.
\end{equation}
Using this, a finite volume discretization of \eqref{eq:RTEa} when $\epsilon = 1$ and $\sigma_{\rm{s}}=\sigma_{\rm{t}}-\sigma_{\rm{a}}$ is
\begin{equation}
\frac{\Omega_{k,x}}{\Delta x_i}\left(\psi_{k,i+1/2,j} - \psi_{k,i-1/2,j}\right) + \frac{\Omega_{k,y}}{\Delta y_j}\left(\psi_{k,i,j+1/2} - \psi_{k,i,j-1/2}\right) + \sigma_{\rm{t}}\psi_{k,i,j} = \frac{\sigma_{\rm{s}}}{4\pi}\phi^N_{i,j}+q_{i,j},
\end{equation}
where $\phi^N_{i,j}$ and $q_{k,i,j}$ are the cell averages of $\phi^N(x,y)$ and $q_k(x,y)$ respectively. Suppose $\psi_k(x,y)$ is nearly a linear function of $x$ and $y$ across the cell, such that
\begin{equation}
    \psi_k(x,y)\approx \psi_{k,i,j} + s_{k,x_i}(x-x_i) + s_{k,y_j}(y-y_j),\quad |x-x_i|\le \Delta x_i/2,\ |y-y_j|\le \Delta y_j/2,
\end{equation}
where $s_{k,x_i}$ and $s_{k,y_j}$ are slopes to be determined. Using an upwind scheme, we make the following choices:
\begin{align}
    \psi_{k,i+1/2,j} &= \psi_{k,i,j} + s_{k,x_i}\Delta x_i/2,\quad \Omega_{k,x}>0,\\
    \psi_{k,i-1/2,j} &= \psi_{k,i,j} - s_{k,x_i}\Delta x_i/2,\quad \Omega_{k,x}<0,\\
    \psi_{k,i,j+1/2} &= \psi_{k,i,j} + s_{k,y_j}\Delta y_j/2,\quad \Omega_{k,y}>0,\\
    \psi_{k,i,j-1/2} &= \psi_{k,i,j} - s_{k,y_j}\Delta y_j/2,\quad \Omega_{k,y}<0,\\
\end{align}
where
\begin{equation}
    s_{k,x_i}=\begin{cases}
    \frac{2\psi_{k,i,j}}{\Delta x_i},\quad i=1,\ \Omega_{k,x}>0\\
    \frac{\psi_{k,i,j}-\psi_{k,i-1,j}}{\Delta x_i},\quad i>1,\ \Omega_{k,x}>0\\
    \frac{\psi_{k,i+1,j}-\psi_{k,i,j}}{\Delta x_i},\quad i<I,\ \Omega_{k,x}<0\\
    \frac{-2\psi_{k,i,j}}{\Delta x_i},\quad i=I,\ \Omega_{k,x}<0
    \end{cases}
\end{equation}
\begin{equation}
    s_{k,y_j}=\begin{cases}
    \frac{2\psi_{k,i,j}}{\Delta y_j},\quad j=1,\ \Omega_{k,y}>0\\
    \frac{\psi_{k,i,j}-\psi_{k,i,j-1}}{\Delta y_j},\quad j>1,\ \Omega_{k,y}>0\\
    \frac{\psi_{k,i,j+1}-\psi_{k,i,j}}{\Delta y_j},\quad j<J,\ \Omega_{k,y}<0\\
    \frac{-2\psi_{k,i,j}}{\Delta y_j},\quad j=J,\ \Omega_{k,y}<0
    \end{cases}
\end{equation}
